Learning Generalizable Program and Architecture Representations for Performance Modeling

Performance modeling is an essential tool in many areas, including performance characterization/optimization, design space exploration, and resource allocation problems, to name a few. However, existing performance modeling approaches have limitations, such as high computational cost for discrete-event simulators, narrow flexibility of hardware emulators, or restricted accuracy/generality of analytical/data-driven models. To address these limitations, this paper proposes PerfVec, a novel deep learning-based performance modeling framework that learns high-dimensional and independent/orthogonal program and microarchitecture representations. Once learned, a program representation can be used to predict its performance on any microarchitecture, and likewise, a microarchitecture representation can be applied in the performance prediction of any program. Additionally, PerfVec yields a foundation model that captures the performance essence of instructions, which can be directly used by developers in numerous performance modeling related tasks without incurring its training cost. The evaluation demonstrates that PerfVec is more general and efficient than previous approaches.

==> Makefile <==
MAINFILE = main.tex

PDF = ${MAINFILE:%.tex=%.pdf}


all:  ${PDF}

ad:  sc24_ad_ae.pdf

%.pdf:  %.tex content/*.tex fig/*.pdf *.bib
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

clean:
	$(RM)  *.log *.aux *.pdf \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi


==> content/comparison.tex <==
\secspace
\section{Comparison of Performance Modeling Methodologies}
\label{sect:comparision}
\secspace

\begin{table*}[t]
\centering
%\footnotesize
\scriptsize
%\tiny
\caption{Comparison of performance modeling methodologies.}
\label{tbl:comparison}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\bf \minitab[c]{Performance modeling\\ methodology}} & \multirow{2}{*}{\bf Prerequisite} & \multicolumn{2}{c|}{\bf Overhead} &  \multirow{2}{*}{\bf Accuracy} &  \multirow{2}{*}{\bf Generality} \\
\cline{3-4}
 & & {\bf Preparation} & {\bf Prediction} & & \\
\hline
\hline
\minitab[c]{Human-engineered analytical\\ modeling \cite{CACM09:Roofline, TOCS09:Eyerman, TC16:Steen}} & \minitab[c]{Construct models and\\ profile programs} & Medium & Very fast & Low & Varies \\
\hline
\minitab[c]{ML-based analytical\\ modeling \cite{ASPLOS06:Ipek, HPCA07:Lee}} & \minitab[c]{Acquire training data for target\\ programs and \uarchs\\ through simulation, etc.} & Slow & Very fast & Varies & Low \\
\hline
Cycle-accurate simulation \cite{gem5} & Implement simulator modules & Medium & Slow & Medium & High \\
\hline
ML-based simulation \cite{SIGMETRICS22:simnet} & \minitab[c]{Acquire training data for\\ target \uarchs} & Slow & Medium & Medium & Medium \\
\hline
Emulation \cite{MICRO07:Chiou, ISCA18:FireSim} & Implement \& verify RTL modules & Very slow & Fast & Varies & Medium \\
\hline
\pv & \minitab[c]{Acquire program and/or\\ \uarch \repse} & Medium & Very fast & Medium & High \\
\hline
\end{tabular}
\end{table*}

%\subhead{Comparison with State-of-the-Arts.}
Table \ref{tbl:comparison} summarizes all performance modeling methodologies,
including \pve.
%While this section focuses on the comparison of methodologies, Section
%\ref{sect:relatedwork} will introduce individual approaches in more detail.
They are compared based on the prerequisite effort, time
overhead, accuracy, and generality.
The time overhead is further divided into the time to prepare the model and to
make prediction.

% Comparison.
Human-engineered analytical models are widely used due to their simplicity and
lighting-fast prediction speed.
They also provide more insights compared with ML-based models because they are
built explicitly.
Yet, because of the complexity of modern processors, they often fall short on
accuracy.
For generality, both general and program/\uarche-specific models have been
introduced in the past \cite{CACM09:Roofline, TOCS09:Eyerman,
Computer09:Barker, ICS14:Palm}.
More general models tend to sacrifice further in terms of accuracy.
%e.g., the Roofline model \cite{CACM09:Roofline}.
Compared with these models, \pv has better generality and accuracy without speed loss.

To compensate for the accuracy loss in human-engineered analytical models,
ML-based analytical models have been proposed to exploit the excellent
function approximation ability of ML models.
The major limitation of existing ML-based models is they are program- and
\uarche-specific, i.e., having low generality.
As a result, slow training data acquisition is needed whenever target programs
or \uarchs change, significantly limiting their practicality.
Section \ref{sect:case:dse} has illustrated that \pv achieves faster design
space exploration due to its better generality.
%Compare with ML-based application level models: workflow advantage; knowledge
%reuse; unseen programs; one program one data point vs. many data points in
%training data acquisition...
%Training cost: instruction level vs. program level.

Cycle-accurate simulation is the default performance modeling approach used by
hardware designers in early stages.
Modern simulation frameworks are flexible in executing different programs,
changing the configurations, and adding new modules.
The major drawback of simulation is the speed.
Simulating real-world programs can take several months/years.
Thus, they are
often used together with mini-applications, reduced inputs, and/or simulation reduction
techniques \cite{ASPLOS02:SimPoint, SIGMETRICS03:SimPoint}.

Recently, ML-based simulators have been introduced to accelerate simulation using
GPUs.
Although they are \gbl across different programs, they remain \uarche-dependent.
Compared with them, \pv is both program- and \uarche-independent.
It also makes prediction much faster because program \reps are reusable, while
ML-based simulators need to go through all instructions one by one.

Hardware emulators, such as field-programmable gate arrays (FPGAs), can execute programs and evaluate their
performance in the native hardware speed.
They can be precise when implemented in the same way as the target design.
%Hardware constraints can impact he accuracy of emulators, e.g., FPGA logic and
%memory frequency limitations.
The main drawback to emulation is that register-transfer level (RTL) implementation and verification are
extremely time consuming, requiring at least several human years.
Furthermore, this expensive process needs to repeat whenever the target \uarch
changes.

%Time cost (data acquisition, training), human efforts, model reuse...
%When having new programs, when having new \uarchs...
%Section \ref{} compares our \repe-based modeling with simulation and existing
%ML-based analytical modeling in the design space exploration setting.

%Whole program representation: graph model not capable.
%Capable of dealing with real-world programs.
%GNNs can only address limited sized programs since messages are passed among
%instruction nodes, while \pv can handle arbitrarily large programs.

% Interpretability
%Explain different positions in the learned representation: some may relate to cache, memory, etc.
%Through average gradient on inputs?
%Memory intensity as a combination of representations.

In summary, the advantages of \pv are its generality and low overhead compared
with other performance modeling approaches.
% Where generality comes from.
Due to the composability of instruction \repse, \pv generalizes to all
programs compiled on the same ISA.
\pv also generalizes to unseen \uarchs because it is trained using random
\uarch samples.
Moreover, users incur low overhead with \pve, because the program and \uarch
\reps are \gbl and reusable, and they can leverage pre-trained instruction
\rep models to generate \reps for new programs.
While our evaluation shows that \pv achieves sufficient accuracy, we believe it
can be further improved with larger training datasets, as well as more extensive
ML model searches.
%It only have some accuracy disadvantages compared with certain non-\gbl
%ML-based analytical models.
%We believe contiguous training on larger datasets and further model exploration
%will eventually close the accuracy gap.

One limitation of \pv is that the resultant instruction \rep model is
ISA-dependent.
This paper details our work of training instruction \rep models for the ARMv8
ISA, which dominates the mobile and embedded markets and continues to grow in
the PC and server markets.
There are only a few other popular ISAs in the world, such as x86
and RISC-V.
It is straightforward to apply the technique proposed in this work to train, for example, an x86 instruction \rep model.
We leave \rep models for other ISAs as potential future work.

